SIMMC 2.0: A Task-oriented Dialog Dataset for Immersive Multimodal Conversations

Next generation task-oriented dialog systems need to understand conversational contexts with their perceived surroundings, to effectively help users in the real-world multimodal environment. Existing task-oriented dialog datasets aimed towards virtual assistance fall short and do not situate the dialog in the user's multimodal context. To overcome, we present a new dataset for Situated and Interactive Multimodal Conversations, SIMMC 2.0, which includes 11K task-oriented user<->assistant dialogs (117K utterances) in the shopping domain, grounded in immersive and photo-realistic scenes. The dialogs are collected using a two-phase pipeline: (1) A novel multimodal dialog simulator generates simulated dialog flows, with an emphasis on diversity and richness of interactions, (2) Manual paraphrasing of the generated utterances to collect diverse referring expressions. We provide an in-depth analysis of the collected dataset, and describe in detail the four main benchmark tasks we propose. Our baseline model, powered by the state-of-the-art language model, shows promising results, and highlights new challenges and directions for the community to study.

==> archive/archive_simmc_proposal.tex <==



\section{Motivation}

% 1. Brief recap of SIMMC 1.0
The Situated and Interactive Multimodal Conversaitional AI (SIMMC) challenge \cite{moon2020situated}, held as part of DSTC9 \cite{dstc9}, aimed to lay the foundations for the real-world assistant agents that can handle multimodal inputs, and perform multimodal actions.
Specifically, it provided the SIMMC corpora as a new benchmark dataset for studying task-oriented dialogs that encompass a situated multimodal user context in the form of a co-observed image or virtual reality (VR) environment.
The earlier SIMMC challenge saw a number of model submissions from participants, 
establishing a new set of state-of-the-art baselines for the multimodal task-oriented dialog systems on the SIMMC dataset.

% 2. Building upon it, we propose SIMMC 2.0, addressing the gaps
Building upon the success of the first SIMMC challenge \cite{moon2020situated}, we propose the Second SIMMC Challenge for the community to tackle and continue the effort towards building a successful multimodal assistant agent.
Specifically, we provide the newly collected dataset (SIMMC 2.0) designed to include a closer-to-real-world context for a fashion or furniture shopping scenario, moving away from the sanitized contexts present in the original SIMMC datasets.
To this end, SIMMC 2.0 presents assistant$\leftrightarrow$user task-oriented dialogs grounded on diverse photo-realistic VR renders of (synthetic) commercial stores.
These renderings include a number of referent items and serves as a proxy for real-world
scenarios.
This new dataset captures several interesting challenges such multimodal dialog state tracking, coreferences (``\textit{directly behind it}”, ``\textit{the one I mentioned}”), and disambiguation (``\textit{grey jacket to the right of the one I mentioned}”).

% 3. Summary; might be too verbose & repetitive so skip
%\textbf{In summary}, SIMMC 2.0 builds upon and extends the previous challenge, addressing the following main key challenges and gaps:
%\begin{itemize}
    %\item More complex multimodal contexts: 
    %\item Multimodal coreference resolution and dialog state tracking: 
    %\item Complex visual scenes: visually challenging problem
%\end{itemize}

%---------------------------------
\begin{figure}[t]
  \centering \includegraphics[width=1.0\columnwidth]{figures/overview.png}
  \vspace{-12pt}
  \caption{Illustration of a Situated Interactive Multimodal Conversation (SIMMC), which presents a task-oriented user$\leftrightarrow$assistant dialog grounded in a co-observed multimodal context. The newly collected SIMMC 2.0 dataset includes complex and photorealistic multimodal contexts, which poses more challenges for the Multimodal Coreference Resolution task (MM-Coref) and the Multimodal Dialog State Tracking task. } 
  \label{fig:teaser}
  \vspace{-10pt}
\end{figure}
%---------------------------------


\section{SIMMC Challenge 2.0}

We now detail the new multimodal conversational dataset (\refsec{subsec:dataset}) and propose 
three main sub-tasks for the challenge (\reftab{tab:tracks}, \refsec{subsec:tracks}).

\subsection{Problem Setup}

%\todo{paraphrase a bit more to avoid self-plagiarism}
The SIMMC challenge addresses the conversational scenarios where the virtual assistant shares a co-observed scene with a user in addition to the traditional communication that takes place in the form of natural language.
Following the SIMMC 1.0 dataset, we choose shopping experience as the domain for this study, as it often induces rich multimodal interactions around browsing visually grounded items.
We assume that the assistant agent has ground-truth meta information of every object in the scene, while users only observe those objects through the visual modality to describe and compose a request.
In addition, we allow users to physically navigate within each scene, which we simulate as multiple viewpoints updated at different time steps throughout each dialog.
Thus, entries to the SIMMC challenge 2.0 would need to understand the user utterance using both the dialog history and the state of the environment as multimodal context.

Note that our problem setup for co-observing assistant scenarios allows for more natural multimodal coreferences to be used as part of user-assistant conversations.
The existing literature in multimodal dialogs \cite{avsd-dstc7,avsd-dstc8,visdial,clevr-dialog,guesswhat,talk-the-walk} often posits the roles of a primary and secondary observer, \ie \textit{questioner} and \textit{answerer} similar to the Visual Question Answering \cite{vqa} tasks, hence showing a different distribution of language.
Our setup also extends many of the challenges studied in the previous literature on task-oriented dialog systems \cite{dstc2, sgd-dst, multiwoz, multiwoz2.1} (\eg DST, slot carryovers) to the unique multimodal settings.


\subsection{Description of Dataset}
\label{subsec:dataset}

\begin{table*}[t]
    \begin{center}
        \scalebox{0.9}{
        \setlength\tabcolsep{9pt}
        \begin{tabular}{p{0.28\textwidth}p{0.35\textwidth}p{0.25\textwidth}}
        \toprule[\heavyrulewidth]
        \textbf{Task Name}  & \textbf{Goal} & \textbf{Evaluation} \\
        \midrule
        1. Multimodal Coreference Resolution & Given user utterances with object mentions, resolve referent objects to their canonical ID(s) as defined by the catalog. & Coref Precision / Recall / F1 \\        
        \midrule        
        2. Multimodal Dialog State Tracking & Given user utterances, track user belief states across multiple turns. & Intent Accuracy,
Slot Precision / Recall / F1 \\
        \midrule
        3. Response Generation & Given user utterances, ground-truth APIs and ground-truth object IDs, generate Assistant responses or retrieve from a candidate pool. & Generation: BLEU, Perplexity, Human Evaluation (Naturalness, etc.); Retrieval: Accuracy@k, Entropy \\
        \bottomrule[\heavyrulewidth]
        \end{tabular}
        }
    \end{center}
    \vspace{-6pt} 
    \caption{\textbf{Proposed tracks and descriptions}}
    \vspace{-8pt} 
    \label{tab:tracks}
\end{table*}


The SIMMC 2.0 dataset assumes the scenario where a user is interacting with a conversational assistant to obtain recommendations for a furniture or a fashion item.
The dialogs were collected through a two-phase pipeline (multimodal dialog simulation \& manual human paraphrase), minimizing the annotation overheads (time and cost).
This approach extends the popular machine$\leftrightarrow$human collaborative dialog collection approaches \cite{sgd-dst, shah2018building} to the multimodal settings.

\textbf{Phase 1}: We generate synthetic dialog flows using a dialog simulator that conditions on various VR scenes for fashion and furniture, produced by a scene simulator.
The scene simulator generates a diverse set of scene snapshots that serve as multimodal context for the conversations. This is done using publicly available digital assets, re-arranging them programmatically at random to create scenes, and capturing a view from a random camera position within the scene. 

The dialog simulator then takes these generated scenes along with the meta information (objects, locations, and attributes) to create a dialog flow between a user and an assistant, following an agenda-based dialog simulator approach \cite{schatzmann2007agenda}.
Each agenda describes a high-level sequence of shopping scenarios (\eg \texttt{BROWSE} $\rightarrow$ \texttt{GET\_INFO} $\rightarrow$ \texttt{REFINE}).
The simulated dialog flows consist of NLU/NLG intents (\eg \texttt{REQUEST:GET}, \texttt{CONFIRM:ADD\_TO\_CART}), slots (\eg color, pattern), and object references, following the ontology developed for SIMMC 1.0 \cite{moon2020situated}.

\textbf{Phase 2}: The simulated dialog flows are then paraphrased by human annotators. This helps us draw utterances from the natural language distribution, as expected in a real world application. For this annotation effort, we designed a tool that displays a multimodal scene (generated VR scene screenshot) and a simulated dialog flow, and asked the human annotators to paraphrase the utterance ensuring that critical information such as objects and attributes is retained. An example dialog is shown in \reffig{fig:example}.

\begin{table}[h]
    \begin{center}
        \scalebox{0.92}{
        \begin{tabular}{lccc}
        \toprule[\heavyrulewidth]
        Total \# dialogs & 11,244 \\
        Total \# utterances & 117,236 \\
        Total \# scenes & 3,133 \\
        Avg \# words per user turns 	& 12 \\
        Avg \# words per assistant turns &	13.7 \\
        Avg \# utterances per dialog 	& 10.4 \\
        Avg \# objects mentioned per dialog &	4.7 \\
        Avg \# objects in scene per dialog &	19.7 \\
        \bottomrule[\heavyrulewidth]
        \end{tabular}
        }
    \end{center}
    \vspace{-10pt} 
    \caption{\textbf{SIMMC 2.0 Dataset Statistics}}
    \vspace{-10pt}   
    \label{tab:datasets_statistics}
\end{table}

We collected a total of 11,244 dialogs (117,236 utterances), with the fine-grained ground-truth dialog labels (NLU/NLG/Coref) already in place.
Table~\ref{tab:datasets_statistics} shows the statistics of the dataset.

\noindent
\textbf{Differences between SIMMC 1.0 and 2.0}.
The key differences are (illustrated in \reffig{fig:teaser}):

\noindent
(a) The multimodal context in SIMMC 1.0 consists of either co-observed images or VR environment,
which are simplistic and sanitized in comparison to real-world scenarios.
For instance, the VR environment in SIMMC-Furniture comprises three slots (left, center, right) 
to populate the catalog items, thus limiting the complexity of referential or disambiguation language.
In contrast, conversations in SIMMC 2.0 are grounded in photo-realistic scene renderings of
commercial stores that are cluttered and thus closely represent the real-world contexts.

\noindent
(b) The number of objects in the multimodal context for SIMMC 1.0 at any turn is capped at 3
compared to $19.7$ on average for SIMMC 2.0.
This allows for richer coreferences, referential expressions, and disambiguation scenarios, 
elevating the role of dialog.

\noindent
(c) Many of the objects in each scene are only partially observed (\eg, blocked by different items or shelves, out of POV frame), which reflects real-world scenes but poses a more challenging problem for the computer vision module.

\noindent
\textbf{Data format}:
The SIMMC 2.0 data will be provided in the similar format as the earlier version of the dataset, to make it easier for participants to leverage the benchmark models publicly available \cite{moon2020situated}, or augment it with the previous version of the dataset for pretraining, etc.
The raw pixel images of each scene as well as the pre-computed visual embeddings (via a popular CV model) will be provided, to make it easier to use the dataset.

\subsection{Challenge Tasks}
\label{subsec:tracks}

We invite participants to model multimodal conversational agents adept at replicating humans for this dataset and enable deep shopping scenarios as a result.
The entries to the SIMMC 2.0 challenge would thus need to have a strong computer vision capability to consume raw images we provide, and a multimodal conversational reasoning capability to understand both the dialog and the visual contexts. 
Specifically, we propose three sub-tasks and evaluation metrics addressing the challenges in the multimodal conversational reasoning (summarized in \reftab{tab:tracks}).
A script for calculating these metrics will be provided with the dataset.

\subsubsection{Multimodal Coreference Resolution (MM-Coref)}
For this task, we aim to resolve referential mentions in user utterances to their canonical object IDs as defined for each scene.
These mentions can be resolved through (1) the dialog context (\eg A: ``\textit{\underline{This shirt} comes in XL and is \$29.}" $\rightarrow$ U: ``\textit{Please add \underline{it} to cart.}", or (2) the multimodal context (\eg U: ``\textit{How much is that \underline{red shirt}?}"), or (3) both (\eg U: ``\textit{How much is \underline{the one} next to \underline{the one you mentioned}?}").

Participants will be provided with ground-truth bounding boxes defining each object ID.
The performance will mainly be measured for its F1 score.

\subsubsection{Multimodal Dialog State Tracking (MM-DST)}
Following the earlier challenge, we extend the traditional notion of the unimodal dialog state tracking (DST) problem and propose MM-DST as a main sub-task where slots are grounded on the coexisting multimodal context, which requires handling of multimodal objects (as opposed to textual tokens) as part of dialog states.

\subsubsection{Assistant Response Generation}
The goal of this task is to generate Assistant responses or retrieve from a candidate pool, given user utterances, ground-truth APIs and object IDs.
While we assume the assistant agent has the ground-truth meta information on each object, each response needs to naturally describe the referent objects \textit{as observed and understood} by the user through the co-observed scene or the dialog context (\eg \texttt{INFORM:RECOMMEND (OBJ\_ID: 3)} $\rightarrow$ A: ``\textit{I recommend the blue shirt directly behind the brown jacket.}". 


\section{Organizers}

\noindent Seungwhan Moon; \texttt{shanemoon@fb.com}

\noindent Satwik Kottur; \texttt{skottur@fb.com}

\noindent Paul A. Crook; \texttt{pacrook@fb.com}

\noindent Ahmad Beirami; \texttt{beirami@fb.com}

\noindent Eunjoon (EJ) Cho; \texttt{ejcho@fb.com}

\noindent Babak Damavandi; \texttt{babakd@fb.com}

\noindent Alborz Geramifard; \texttt{alborzg@fb.com}

\noindent Rajen Subba; \texttt{rasubba@fb.com}


\bibliography{bibliography}
\bibliographystyle{plain}
% \bibliographystyle{acl_natbib}
\vfill
\pagebreak

\input{tex/supplementary.tex}


==> archive/sections/dataset.tex <==

%---------------------------------
\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\columnwidth]{figures/multiple_scenes.png}
    \caption{
    Example snapshots from random camera viewpoints generated from a rearranged scene.
    Refer to \refsec{sec:scene_simulator} for more details.
    }
    \label{fig:scene_generator_examples}
\end{figure}
%---------------------------------

%---------------------------------
\begin{figure*}[t]
  \centering \includegraphics[width=1.9\columnwidth]{figures/data_collection.png}
  %\vspace{-12pt}
  \caption{Illustration of the two-stage data collection pipeline. \smtodo{expand} Phase 1: Simulated Multimodal Dialog Self-Play (\refsec{subsec:dataset:phase1}) \& Phase 2: Manual Human Paraphrase (\refsec{subsec:dataset:phase2})} 
  \label{fig:data_collection}
  %\vspace{-10pt}
\end{figure*}

The \dn{} dataset assumes the scenario where a user is interacting with a 
conversational assistant to obtain recommendations for a furniture or a fashion item.
The dialogs were collected through a two-phase pipeline (\reffig{fig:data_collection}), 
minimizing the annotation overheads (time and cost).
This approach extends the popular machine$\leftrightarrow$human collaborative dialog collection approaches \cite{sgd-dst, shah2018building} to the multimodal settings.

\subsection{Multimodal Dialog Self-Play}
\label{subsec:dataset:phase1}

\sk{
The first phase entails generating synthetic dialog flows between the user and 
assistant using a multimodal dialog simulator (\refsec{sec:dialog_simulator}).
The simulator conditions the flow generation on various VR scenes snapshots for 
both fashion and furniture domains.
These snapshots are produced by a scene simulator that we describe next.
}
\subsubsection{Scene Simulator}
\label{sec:scene_simulator}
\sk{
In our work, we use photo-realistic, virtual renderings of cluttered shopping
environments for fashion and furniture domains, to replicate real-world settings.
To this end, we develop a scene simulator to generate a diverse set of snapshots
that serve as the multimodal context for the conversations.
}

\noindent
\textbf{Scene Generation.}
\sk{
Rearranging objects in a 3D semantically to create novel arrangements is a long standing
research problem \cite{2012-scenesynth,fisher2015actsynth}.
To avoid the challenges in a completely automatic approach, we design the following pipeline
in a VR environment \cite{unitygameengine}.
We begin by manually constructing photo-realistic shopping scenarios as `seed scenes',
using publicly available digital assets like,
(a) fashion: shirts, dresses, trousers, and shoes,
(b) furniture: sofas, chairs, dining table, and lamps.
We then programmatically re-arrange these assets at random for each of these seed
scenes to create a larger pool of scenes (\reftab{tab:datasets_statistics}),
while keeping the semantics of the scene intact.
For example, a shirt in the seed scene is replaced only by another asset from either the 
same (shirt) or semantic related asset category (\eg, T-shirt, jacket).
This ensures that re-arranged scenes continue to be photo-realistic and avoids object 
collisions and hallucinations, trading off with fixed arrangement
of semantic asset types within each seed scene.
}

\sk{
Finally, we capture multiple views from random camera position within each scene,
as shown in \reffig{fig:scene_generator_examples}.
The height of the camera is mostly held constant with a small jitter, whereas the 
camera position (when projected onto the floor plane) is randomly chosen and is constrained
to be within $75\%$ of the floor bounds.
These settings give us a good view of the scene objects without the risk of being either:
(a) too close, such that entire snapshot is taken by partially visible 1--2 objects
resulting in a poor and uninteresting scene view, or,
(b) too far away, where objects are small and hard to differentiate from one another.
Randomly sampled camera viewpoints also encourage the diversity of referring expressions 
(\eg, \textit{`shirt closest to the changing rooms'}, 
\textit{`cap at the farthest end of the table'}),
useful for successful coreferences or disambiguation within the dialog utterances.
}

\noindent
\textbf{Annotation Extraction.}
\sk{
The synthetic nature of our scenes facilitates an easy extraction of complete scene graph 
information for any given snapshot, without any additional human annotations.
This is particularly beneficial as it enables the generation of rich and interesting dialog 
flows (\refsec{sec:dialog_simulator}),
and allows for a tighter control over the distribution of objects and attributes within 
the conversation, which is nearly impossible with real world multimodal contexts.
The annotations we extract for each scene snapshot consists of all the assets that appear in
the snapshot, their image 2D bounding box, and an index to cross reference additional 
metadata from the catalog (\eg, price, available sizes, color, pattern).
After extracting these annotations, we filter out snapshots with less than 5 objects in 
field of view, and input the remaining to the multimodal dialog simulator.
See \refsec{sec:dataset_analysis} for a detailed analysis of the generated scene snapshots 
and the underlying assets used in our work.
}


\subsubsection{Multimodal Dialog Simulator}
\label{sec:dialog_simulator}

The multimodal dialog simulator takes these generated scenes along with the meta information (objects, locations, and attributes) to create a dialog flow between a user and an assistant, following an agenda-based dialog simulator approach \cite{schatzmann2007agenda}.
\sm{
\noindent 
\textbf{Multimodal Dialog Self-play.}
The dialog simulator consists of three main components: the \textit{goal generator}, the \textit{user simulator}, and the \textit{assistant simulator}.
The goal generator randomly selects an agenda for each dialog, which describes a high-level sequence of \textit{goals} within shopping scenarios (\eg, \texttt{BROWSE} $\rightarrow$ \texttt{GET\_INFO} $\rightarrow$ \texttt{REFINE}; 
see \reffig{fig:fashion_act_transitions}).
Given a goal, the user simulator draws a suitable dialog action following a probability distribution, which consists of natural language understanding (NLU) intents (\eg, \texttt{REQUEST:GET}, \texttt{CONFIRM:ADD\_TO\_CART}), 
slots (\eg, color, pattern), and object references.
The assistant simulator then reads the user request, interacts with the multimodal contexts via the simulated API (\eg for looking up the information of an item from the catalog, recommending items from the scene), and responds with a natural language generation (NLG) intents, slots and object references.
This dialog self-play repeats until each goal in the agenda is successfully met, or when the dialog reaches the maximum number of turns.
}

\sm{
\noindent
\textbf{Multimodal Dialog Ontology.}
The dialog annotations for \dn{} include the NLU and NLG intent and slot labels, following the conventional approaches for task-oriented dialog systems \cite{multiwoz2.1, sgd-dst, moon2020situated}.
Extending the dialog ontology for the complex multimodal settings, we also annotate the object references with their corresponding IDs as defined by the bounding boxes in each scene, allowing for a seamless annotation of multimodal contexts and language (\eg \textit{`Do you have anything similar to the two middle jackets on the table?'} $\rightarrow$ \texttt{INFORM:GET\_SIMILAR, slots: \{type: jacket\}, objects: [0,8]}).
Note also that the same notation is employed to refer to object mentions that are carried over in the dialog context (\eg \textit{`How much is the jacket I mentioned earlier?'} $\rightarrow$ \texttt{INFORM:GET.price, objects: [8]}).
This fine-grained and unified ontology allows for the systemic study of the diverse referring expressions (\ie object mentions) in multimodal dialogs.  
}


\subsection{Manual Paraphrase}
\label{subsec:dataset:phase2}

\smtodo{expand below}

The simulated dialog flows are then paraphrased by human annotators. This helps us draw utterances from the natural language distribution, as expected in a real world application. For this annotation effort, we designed a tool that displays a multimodal scene (generated VR scene screenshot) and a simulated dialog flow, and asked the human annotators to paraphrase the utterance ensuring that critical information such as objects and attributes is retained. An example dialog is shown in \reffig{fig:example}.

\begin{table}[t]
    \begin{center}
        \scalebox{0.92}{
        \begin{tabular}{lccc}
        \toprule[\heavyrulewidth]
        Total \# dialogs & 11,244 \\
        Total \# utterances & 117,236 \\
        Total \# scene snapshots & 1566 \\
        Avg \# words per user turns 	& 12 \\
        Avg \# words per assistant turns &	13.7 \\
        Avg \# utterances per dialog 	& 10.4 \\
        Avg \# objects mentioned per dialog &	4.7 \\
        Avg \# objects in scene per dialog &	19.7 \\
        \bottomrule[\heavyrulewidth]
        \end{tabular}
        }
    \end{center}
    %\vspace{-10pt} 
    \caption{\textbf{\dn{} Dataset Statistics}}
    %\vspace{-10pt}   
    \label{tab:datasets_statistics}
\end{table}

\textbf{Advantages of the two-stage approach}:
Since paraphrasing synthetic utterances is much faster and less demanding, our approach requires reduced annotation effort. Further, the simulator in Phase 1 provides all annotations for the dialog state and coreferences for free, \ie, without any additional human annotations. 




==> archive/sections/dataset_analysis.tex <==
\sk{
We analyze our dataset that contains a total of $11.2k$ dialogs (about $117k$ utterances),
split into $7.2k$ and $4k$ dialogs from fashion and furniture domains respectively,
along with the rich annotations from both scene simulator and multimodal
dialog simulator that are extracted automatically without any additional human annotators.
\reftab{tab:datasets_statistics} shows the overall statistics of the dataset.
}

\noindent
\textbf{Analyzing Assets \& Scene Snapshots.}
\sk{
% As described in \refsec{sec:scene_simulator}, we manually construct seeds scenes using publicly 
% available digital assets, and rearrange them semantically to result in a larger pool of
% scenes.
In our work, we use around $290$ digital assets for 
fashion\footnote{\url{https://www.turbosquid.com/}}, and
$110$ assets for furniture\footnote{\url{https://www.wayfair.com/}}, across several
asset categories shown in \reftab{tab:simmc_assets}.
From these assets, we construct $7$ seed scenes for fashion and $1$ seed scene for furniture.
We then rearrange assets within each seed scenes $20$ times to result in a pool of $140$ and 
$20$ scenes for respective domains.
Finally, we extract $10$ snapshots from random camera viewpoints for each scene in the pool
giving us a total of about $1566$ unique scene snapshots to choose from post filtering.
The number of objects in each snapshot is distributed as shown in
\reffig{fig:snapshot_asset_distr}.
This huge variance presents a good opportunity for the dialog simulator to ground the 
conversational flow in a varied number of objects.
}

\begin{table*}[th]
    \centering
    \begin{tabular}{l p{5.5in}}
    \toprule
         Fashion &
         hat, tshirt, jacket, hoodie, sweater, shirt, suit, vest, coat, trousers,
         jeans, joggers, skirt, blouse, tank top, dress, shoes \\
         Furniture &
         area rug, bed, chair, couch chair, dining table, coffee table, end table,
         lamp, shelves, sofa \\
    \bottomrule
    \end{tabular}
    \caption{Digital Asset Categories used in \dn{} for both fashion and furniture domains.}
    \label{tab:simmc_assets}
\end{table*}
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{figures/snapshot_asset_distr.png}
        \caption{}
        \label{fig:snapshot_asset_distr}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{figures/snapshot_dialog_distr.png}
        \caption{}
        \label{fig:snapshot_dialog_distr}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/utterance_len_distr.png}
        \caption{}
        \label{fig:utterance_len_distr}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/dialog_act_distr.png}
        \caption{}
        \label{fig:dialog_act_distr}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/coreference_distance_distr.png}
        \caption{}
        \label{fig:coreference_distance_distr}
    \end{subfigure}
    \caption{Distribution of 
    (a) number of assets in each snapshot,
    (b) number of dialogs for each snapshot,
    (c) utterance lengths with dialog turns,
    (d) acts and activities, and
    (e) coreference distance between object mentions.}
\end{figure*}

\noindent
\textbf{Analyzing Dialog Annotations.}
\sk{
The dialog simulator generates dialog flows by randomly sampling from the pool of 
$1566$ filtered snapshots, which are later manually paraphrased.
While most of the dialogs ($9.3k$) are grounded in a single snapshot, we include few dialog
flows that spans over two snapshots ($1.9k$) with overlapping set of objects. 
This allows for modeling interesting conversations that require a context carry-over 
across the two viewpoints, thus moving closer to the real-world scenario.
Each snapshot corresponds to about $7.1$ dialogs on an average with the distribution
shown in \reffig{fig:snapshot_dialog_distr}.
Further, each dialog contains around $5.2$ utterance pairs (user$\leftrightarrow$assistant), 
where the utterances are $12.0$ and $13.7$ tokens long respectively
(see \reffig{fig:utterance_len_distr} for distribution over different turns).
}

\sk{
Following prior work \cite{moon2020situated}, our dialog annotations also comprise 
dialog acts ($4$: \texttt{INFORM}, \texttt{CONFIRM}, \texttt{REQUEST}, \texttt{ASK}) and 
activities ($5$: \texttt{GET}, \texttt{DISAMBIGUATE}, \texttt{REFINE},
\texttt{ADD\_TO\_CART}, \texttt{COMPARE}).
\reffig{fig:dialog_act_distr} shows their frequency breakdown.
We also visualize the dialog act transitions for furniture in
\reffig{fig:fashion_act_transitions} for the first four rounds of the dialog.
The presence of wide branch-offs and inter-connectivity suggests that our simulator is able 
to generate a diverse set of flows, useful to train a robust conversational system.
It is interesting to note that the user utterances (marked with :U) almost always are more
varied than assistant counterparts (marked with :A).
This is probably due to \texttt{INFORM:GET} (fetching information) being a reasonable assistant
response to a large number of user utterance queries.
Finally, \reffig{fig:coreference_distance_distr} shows the challenging nature of
coreferences within our dialogs, where we measure the distance to the latest mention of
an object, and requires models to reason across the utterances.
}

% \FIXME{\#slots, values, coreference distances, disambiguation statistics}
% \FIXME{Transition plots?}
% \FIXME{furniture}
% {4: 100.0}
% fashion
% {5: 73.72998343456653, 7: 12.203202650469354, 10: 7.647708448371065, 9: 6.419105466593042}}
% Dialog Acts: {'INF', 'CON', 'REQ', 'ASK'}
% Activities: {'GET', 'DIS', 'REF', 'ADD', 'COM'}

\begin{figure*}
    \centering
    \includegraphics[width=0.99\textwidth]{figures/fashion_sankey.png}
    \caption{
    \sk{
    Dialog act transitions for the first four rounds of dialogs in the fashion domain.
    Label \texttt{ACT:ACTIVITY:[A$|$U][turn]} denotes the act and activity 
    (shortened for brevity; see \reffig{sec:dataset_analysis} for full names),
    either \textbf{A}ssistant or \textbf{U}ser utterance with turn index.
    The wide branch-offs and inter-connectivity demonstrates the diversity of dialog
    flows generated by our dialog simulator.
    }}
    \label{fig:fashion_act_transitions}
\end{figure*}


\subsection{Comparison: SIMMC 2.0 vs SIMMC 1.0}
The key differences between \dn{} (ours) and SIMMC 1.0 \cite{moon2020situated}
are (also illustrated in \reffig{fig:teaser}):

\noindent
(a) The multimodal context in SIMMC 1.0 consists of either co-observed images or VR environment,
which are simplistic and sanitized in comparison to real-world scenarios.
For instance, the VR environment in SIMMC-Furniture comprises three slots (left, center, right) 
to populate the catalog items, thus limiting the complexity of referential or disambiguation language.
In contrast, conversations in \dn{} are grounded in photo-realistic scene renderings of
commercial stores that are cluttered and thus closely represent the real-world contexts.

\noindent
(b) The number of objects in the multimodal context for SIMMC 1.0 at any turn is capped at 3
compared to $19.7$ on average for \dn.
This allows for richer coreferences, referential expressions, and disambiguation scenarios, 
elevating the role of dialog.

\noindent
(c) Many of the objects in each scene are only partially observed (\eg, blocked by different items or shelves, out of POV frame), which reflects real-world scenes but poses a more challenging problem for the computer vision module.



\begin{table*}[t]
    \begin{center}
        \scalebox{0.9}{
        \setlength\tabcolsep{9pt}
        \begin{tabular}
        {p{0.20\textwidth} p{0.44\textwidth} p{0.34\textwidth}}
        
        \toprule[\heavyrulewidth]
        \textbf{Task Name}  & \textbf{Goal} & \textbf{Evaluation} \\
        \midrule
        %1. Multimodal Disambiguation & \todo{fill} & Ambiguity Detection Precision / Recall / F1 \\
        %\midrule      
        
        1. Multimodal Disambiguation 
        & Given user utterances, classify if the assistant should disambiguate in the 
        next turn.
        & Binary classification accuracy \\
        
        \midrule
        
        2. Multimodal Coreference Resolution & 
        Given user utterances with object mentions, resolve referent objects to their
        canonical ID(s) as defined by the catalog. 
        & Coref Precision / Recall / F1 \\
        
        \midrule
        
        3. Multimodal Dialog State Tracking 
        & Given user utterances, track user belief states across multiple turns.
        & Intent Accuracy, Slot Precision / Recall / F1 \\
        
        \midrule
        
        4. Response Generation 
        & Given user utterances, ground-truth APIs and ground-truth object IDs, 
        generate Assistant responses or retrieve from a candidate pool.
        & Generation: BLEU, Perplexity, Human Evaluation (Naturalness, etc.); 
        Retrieval: Accuracy@k, Entropy \\
        \bottomrule[\heavyrulewidth]
        \end{tabular}
        }
    \end{center}
    \caption{
    Proposed tasks and descriptions on our \dn{} dataset. 
    Please see \refsec{sec:task_formulation} for more details.
    }
    \label{tab:tracks}
\end{table*}


==> archive/sections/introduction.tex <==
%-------------- Teaser -------------------
\begin{figure}[t]
  \centering \includegraphics[width=0.99\columnwidth]{figures/overview.png}
  % \vspace{-12pt}
  \caption{Illustration of a Situated Interactive Multimodal Conversation (SIMMC), which presents a task-oriented user$\leftrightarrow$assistant dialog grounded in a co-observed multimodal context. The newly collected \dn{} dataset includes complex and photorealistic multimodal contexts, which poses more challenges for the Multimodal Coreference Resolution task (MM-Coref) and the Multimodal Dialog State Tracking task. } 
  \label{fig:teaser}
  % \vspace{-10pt}
\end{figure}
%---------------------------------

% 1. Brief recap of SIMMC 1.0
The Situated and Interactive Multimodal Conversaitional AI (SIMMC) challenge \cite{moon2020situated}, held as part of DSTC9 \cite{dstc9}, aimed to lay the foundations for the real-world assistant agents that can handle multimodal inputs, and perform multimodal actions.
Specifically, it provided the SIMMC corpora as new benchmark datasets for studying task-oriented dialogs that encompass a situated multimodal user context in the form of a co-observed image or virtual reality (VR) environment.
Since the introduction of the dataset, a number of follow-up work \cite{simmc1-team1,simmc1-team2,simmc1-team3,simmc1-team4,simmc1-team5} have established a new set of state-of-the-art baselines for the multimodal task-oriented dialog systems on the SIMMC dataset.

% 2. Building upon it -- introduce SIMMC 2.0, addressing the gaps.
%Building upon the success of   %% for better anonymity 
\sm{
Inspired by the first SIMMC challenge \cite{moon2020situated}, we propose a new multimodal dialog dataset (\dn) for the community to tackle and continue the effort towards building a successful multimodal assistant agent.
Specifically, \dn{} is designed to include a closer-to-real-world context for a fashion or furniture shopping scenario, moving away from the sanitized contexts present in the original SIMMC datasets.
To this end, we propose a VR scene generator that allows for controlling and capturing diverse multimodal contexts with ground-truth scene graph information, while serving as a close proxy for real-world scenarios.
We then collect $11K$ assistant$\leftrightarrow$user task-oriented dialogs ($117K$ utterances) grounded on diverse photo-realistic VR renders of commercial stores ($1.5K$ different scenes).
% Make a claim: To our knowledge, this is the first ___

% 3. Highlight new challenges & the gaps it fills
The incorporation of the complex and cluttered multimodal contexts introduces several interesting challenges, such as understanding visual \textit{and} dialog coreferences (`\textit{the one directly behind it}', `\textit{the one I mentioned}'), tracking dialog states along with multimodal objects, etc.
In addition, the use of photo-realistic scenes surfaces practical limitations of CV models that need to be addressed, such as the detection of partially observed or obstructed referent objects, the visual texture recognition, etc.

% 4. Four main tasks
To this end, we propose four main benchmark tasks that are essential in building a multimodal task assistant: Multimodal Disambiguation, Multimodal Coreference Resolution (MM-Coref), Multimodal Dialog State Tracking (MM-DST), and Response Generation.
We then provide a baseline model trained for these tasks, and highlight the key challenges and future research directions.
}

% 3. Summary; might be too verbose & repetitive so skip
%\textbf{In summary}, SIMMC 2.0 builds upon and extends the previous challenge, addressing the following main key challenges and gaps:
%\begin{itemize}
    %\item More complex multimodal contexts: 
    %\item Multimodal coreference resolution and dialog state tracking: 
    %\item Complex visual scenes: visually challenging problem
%\end{itemize}



% \textbf{The main contributions} are as follows: \todo{expand}
% \begin{itemize}
%     \item Multimodal \& Task-oriented in a virtual environment is novel
%     \item Multimodal dialog simulator
%     \item Call out disambiguation
% \end{itemize}

==> archive/sections/modeling.tex <==


In this section, we perform preliminary empirical analysis and train baselines.
We leave more detailed modeling work for the future.
% \todo{we perform preliminary empirical analysis. further modeling to come next.}
%\subsection{Dataset splits}
% \sktodo{expand}

\noindent \textbf{Dataset split}.
We randomly split the dataset into four sets: train ($65\%$), dev ($10\%$), 
dev-test ($10\%$), and test-std ($15\%$).
We leave the test-std as a held-out hidden set for performing a fair comparison of the developed models. 



\input{tex/tab_results}

\sm{
\noindent \textbf{Notations.}
We denote a \simmc dialog with $N_r$ rounds: $\mathcal{D} = \{(U_i, A_i, M_i, B_i)\}_{i=1}^{N_r}$,
where $U_i$ and $A_i$ are the user and assistant utterances,
$M_i$ is the domain-specific multimodal context,
and $B_i$ is a multimodal belief state represented as a semantic parse of user-side dialog (\ie intent, slot, object references, disambiguation labels), respectively.
At each round $t$, given the current user utterance $U_t$, the dialog history 
$H_t={(U_i, A_i)}_{i=1}^{t-1}$, and the multimodal context $M_t$,
the task is to predict the user belief state $B_t$, as well as the natural language assistant response $A_t$.
}


\noindent \textbf{Baseline.}
We benchmark the dataset by training GPT-2~\cite{radford2019language} based transformer
baselines for MM-Coref, DST, and Response Generation tasks.
The baseline model described here takes as input the dialog context and the flattened
multimodal contexts (as structurally formatted strings) to predict the belief states and
the responses, following the popular causal language model approach \cite{soloist, simpletod}.

\sm{
Note that the proposed baseline uses the ground-truth multimodal contexts provided from the scene generator, instead of consuming raw images as input - as would be the case in the real-world settings.
The model is thus intended to establish the soft oracle performance on the proposed dataset, without being obstructed by underlying computer vision model performances.
We leave the development of the vision incorporated models as future work. 
}


\noindent \textbf{Analysis.}
The results are summrized in Table~\ref{tab:results}
Note that the F1 performance on the multimodal object  coreference resolution task on \dn{} is only at 40.27\%, whereas the best model on SIMMC 1.0 \cite{moon2020situated} achieved 85.9\% on the similar task.
This demonstrates that \dn{} presents more complex and cluttered scenes and thus requires more rigorous visual grounding of multimodal contexts (19.7 objects per dialog on average).
We leave a more detailed error analysis as future work.

==> archive/sections/related_work.tex <==
%\todo{rearrange}


\noindent \textbf{Problem Setup}:
The \dn{} dataset addresses the conversational scenarios where the virtual assistant shares a co-observed scene with a user in addition to the traditional communication that takes place in the form of natural language.
%Following the SIMMC 1.0 dataset, 
Specifically, we choose shopping experience as the domain for this study, as it often induces rich multimodal interactions around browsing visually grounded items.
We assume that the assistant agent has ground-truth meta information of every object in the scene, while users only observe those objects through the visual modality to describe and compose a request.
In addition, we allow users to physically navigate within each scene, which we simulate as multiple viewpoints updated at different time steps throughout each dialog.
Thus, models for \dn{} would need to understand the user utterance using both the dialog history and the state of the environment as multimodal context.

\noindent \textbf{Multimodal Dialog Datasets}:
Note that our problem setup for co-observing assistant scenarios allows for more natural multimodal coreferences to be used as part of user-assistant conversations.
The existing literature in multimodal dialogs \cite{avsd-dstc8,visdial,clevr-dialog,guesswhat,talk-the-walk} often posits the roles of a primary and secondary observer, \ie \textit{questioner} and \textit{answerer} similar to the Visual Question Answering \cite{vqa} tasks, hence showing a different distribution of language.

\sm{
\noindent \textbf{Task-oriented Dialog Systems}:
Many datasets have been developed in the past to support various assistant scenarios (\eg booking hotels, reserving hotels) \cite{dstc2, sgd-dst, multiwoz, multiwoz2.1}, defining many challenges in handling user requests under the unimodal dialog setting.
}
Our setup extends many of these challenges studied in the previous literature on task-oriented dialog systems (\eg DST, slot carryovers) to the unique multimodal settings.

\sm{
The most recent thread in building a task-oriented dialog system is to fine-tune an end-to-end system on a large pre-trained causal language model, which achieves the state-of-the-art performance in many metrics \cite{simpletod, soloist, bert-dst-cmu, bert-dst-alexa, DSTC9_SIMMC}.
We follow this line of work and provide a baseline which extends it to accommodate for the multimodal input.
}


==> archive/sections/task_formulation.tex <==
\sk{
The aim of the SIMMC 2.0 dataset is to emulate futuristic, real-world shopping scenarios
where humans converse with a dialog agent in natural language grounded in a situated
multimodal context.
As a step towards this intelligent conversational agent, we leverage the dialogs and
annotations in our dataset and propose four benchmark tasks (summarized in 
\reftab{tab:tracks}) along with evaluation metrics.
These tasks capture several multimodal conversational reasoning challenges, as elaborated next.
}

\subsection{Multimodal Disambiguation}
\sk{
In a real-world conversation, humans often use shorthands (coreferences) in order to refer
to objects / events that have already been mentioned in the dialog.
While we reserve modeling coreference resolution as a challenging task in 
\refsec{sec:coreference_task},
it is important for the system to recognize ambiguous uses of such coreferences even before
attempting to resolve them.
For example, consider
\textit{`A: The blue trouser is priced at \$45. U: What about \underline{those}?'},
where the phrase \underline{those} could be ambiguous in following situations:
(a) The user refers to a group of trousers without specifying the exact one they have in mind,
(b) The user incorrectly uses a shorthand for a novel pair of trousers not mentioned in the 
dialog due to conversational brevity.
In either cases, identifying the need for disambiguation and responding with 
\textit{`Which one are you talking about? The red or the green pair?'} is a desirable
trait for a robust assistant system.
We formulate the task of multimodal disambiguation to test this ability of the system.
}

\sk{
More concretely, given the dialog history and the current user utterance, multimodal
disambiguation requires the agent to predict a binary label conditioned on the multimodal
context, to indicate the presence of a referential ambiguity in the user utterance.
This label could also be useful for other downstream tasks like assistant response
generation (\refsec{sec:response_generation_task}) in order to continue the conversation 
in a meaningful way. 
We use accuracy to measure and compare model performances for this task.
}

\subsection{Multimodal Coreference Resolution (MM-Coref)}
\label{sec:coreference_task}

For this task, we aim to resolve referential mentions in user utterances to their canonical object IDs as defined for each scene.
These mentions can be resolved through (1) the dialog context (\eg A: \textit{`\underline{This shirt} comes in XL and is \$29.'} $\rightarrow$ U: \textit{`Please add \underline{it} to cart.'}, or (2) the multimodal context (\eg U: \textit{`How much is that \underline{red shirt}?}'), or (3) both (\eg U: \textit{`How much is \underline{the one} next to \underline{the one you mentioned}?'}).

\sm{
The input for this task includes the ground-truth bounding boxes defining each object ID, to avoid the performance bottleneck by the object detection algorithms.
The main evaluation metric includes its F1, precision and recall performance.
Note that we exclude from evaluation the object mentions that are immediately followed by a disambiguation request (\eg \textit{`How much is \underline{the one over there}?' $\leftrightarrow$ \textit{`Which one do you mean?'}}, as they do not provide sufficient descriptions for resolving those coreferences.
}

%---------------------------------
\begin{figure*}[t]
  \centering \includegraphics[width=1.9\columnwidth]{figures/baseline.png}
  %\vspace{-12pt}
  \caption{Illustration of the GPT-2 based baseline, which takes as input the dialog context and the flattened multimodal context, and outputs the belief states as well as the system response.} 
  \label{fig:model_architecture}
  %\vspace{-10pt}
\end{figure*}
%---------------------------------

\subsection{Multimodal Dialog State Tracking (MM-DST)}
Following \cite{moon2020situated}, we extend the traditional notion of the unimodal dialog state tracking (DST) problem and propose MM-DST as a main sub-task where slots are grounded on the coexisting multimodal context, which requires handling of multimodal objects (as opposed to textual tokens) as part of dialog states.

\sm{
The performance is measured by the joint F1, recall and precision performance for the cumulative intent, slot and object reference predictions. 
The underlying reasoning behind this task is that the MM-DST labels will be able to provide sufficient information for a multimodal dialog system to carry out dialog policies and actions, given the detected and resolved items in each multimodal scene.
Therefore, the MM-DST task measures the model's holistic understanding of user requests throughout each dialog, including the disambiguation needs as well as the coreferences.
}

\subsection{Assistant Response Generation}
\label{sec:response_generation_task}

\sk{
The goal of this task is to generate assistant responses or retrieve from a candidate pool, given user utterances, ground-truth belief state, and object IDs.
While we assume the assistant agent has the ground-truth meta information on each object, each
response needs to naturally describe the referent objects \textit{as observed and understood} by
the user through the co-observed scene or the dialog context 
(\eg \texttt{INFORM:RECOMMEND (OBJ\_ID: 3)} $\rightarrow$ A: ``\textit{I recommend the blue shirt directly behind the brown jacket.}".

Similar to \cite{moon2020situated}, we propose two ways to evaluate the performance of
systems for response generation:
(a) As a \textbf{generation} task, where the agent is seen as conditional language
model.
Performance is measured using BLEU-4 score \cite{papineni-etal-2002-bleu} between the
generated response and the ground truth response provided with the dataset.
(b) As a \textbf{retrieval} task, where the agent has to pick the ground truth response 
from a list of candidate responses (generated randomly; unique to each utterance).
We use traditional information retrieval metrics like recall@k ($k=\{1, 5, 10\}$),
mean rank, and mean reciprocal rank for comparing model performances.
}

==> archive/tex/shane_macros.tex <==
\usepackage{graphicx} 
\usepackage{multicol}
% \usepackage{subfigure} 
\usepackage{booktabs} 
\usepackage{algorithm} 
\usepackage{algorithmic} 
\usepackage{color}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{multirow, varwidth}
\usepackage{stfloats} 
\usepackage{verbatim}
\makeatletter
\newif\if@restonecol
\makeatother
\usepackage{xr}
\usepackage[amsmath,thmmarks]{ntheorem}

\def\mathbi#1{\textbf{\em #1}}
\newcommand{\bm}[1]{\boldsymbol{#1}}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\newcommand{\argmin}{\operatornamewithlimits{argmin}}

\usepackage{xspace}
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\st{s.t\onedot} \def\St{\emph{S.t}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother

% For drafts only
\newcommand{\smtodo}[1]{}  % to hide all todos
%\newcommand{\smtodo}[1]{{\color{blue}{\small\bf\sf [Shane TO DO: #1]}}}
%\newcommand{\sm}[1]{{\color{blue}{#1}}}
\newcommand{\sm}[1]{{\color{black}{#1}}}

\newcommand{\sktodo}[1]{}  % to hide all todos
%\newcommand{\sktodo}[1]{{\color{olive}{\small\bf\sf [Satwik TO DO: #1]}}}
%\newcommand{\sk}[1]{{\color{olive}{#1}}}
\newcommand{\sk}[1]{{\color{black}{#1}}}
\newcommand{\FIXME}[1]{{\color{red}{\textbf{#1}}}}

% \newcommand{\todo}[1]{}  % to hide all todos
\newcommand{\todo}[1]{{\color{red}{\small\bf\sf [TO DO: #1]}}}
\newcommand{\anyone}[1]{{\color{yellow}{\small\bf\sf [Anyone: #1]}}}

% Definitions for referring to figure, section, table, equation
% (used uniformly thoughout)
%\newcommand{\reffig}[1]{Fig.~\ref{#1}}
%\newcommand{\refsec}[1]{Sec.~\ref{#1}}
%\newcommand{\reftab}[1]{Tab.~\ref{#1}}

==> archive/tex/simmc_macros.tex <==
\newcommand{\simmc}{SIMMC\xspace}
\newcommand{\furniture}{SIMMC-Furniture\xspace}
\newcommand{\fashion}{SIMMC-Fashion\xspace}
\newcommand{\furniturefull}{SIMMC-Furniture (VR)\xspace}
\newcommand{\fashionfull}{SIMMC-Fashion (Image)\xspace}
\newcommand{\platform}{SIMMC Platform\xspace}
\newcommand{\task}{SIMMC Task\xspace}

% reference to logs of items in each scene
\newcommand{\scenedata}{item appearance logs\xspace}
\newcommand{\SceneData}{Item Appearance Logs}

% reference to 'activities' (previously actions) in annotation
\newcommand{\activity}{activity\xspace}
\newcommand{\Activity}{Activity\xspace}
\newcommand{\activities}{activities\xspace}
\newcommand{\Activities}{Activities\xspace}

% Definitions for referring to figure, section, table, equation
% (used uniformly thoughout)
\newcommand{\reffig}[1]{Fig.~\ref{#1}}
\newcommand{\refsec}[1]{Sec.~\ref{#1}}
\newcommand{\reftab}[1]{Tab.~\ref{#1}}
\newcommand{\refeq}[1]{Eq.~\ref{#1}}
\newcommand{\reportval}[2]{$#1$\footnotesize $\pm #2$}
\newcommand{\reportvalbrief}[2]{#1}

% Space around align environment.
\setlength{\abovedisplayskip}{0pt}
\setlength{\belowdisplayskip}{0pt}
\setlength{\abovedisplayshortskip}{0pt}
\setlength{\belowdisplayshortskip}{0pt}

% for dashed midrules
\usepackage{booktabs,arydshln}
\makeatletter
\def\adl@drawiv#1#2#3{%
        \hskip.5\tabcolsep
        \xleaders#3{#2.5\@tempdimb #1{1}#2.5\@tempdimb}%
                #2\z@ plus1fil minus1fil\relax
        \hskip.5\tabcolsep}
\newcommand{\cdashlinelr}[1]{%
  \noalign{\vskip\aboverulesep
           \global\let\@dashdrawstore\adl@draw
           \global\let\adl@draw\adl@drawiv}
  \cdashline{#1}
  \noalign{\global\let\adl@draw\@dashdrawstore
           \vskip\belowrulesep}}
\makeatother



==> archive/tex/space_saver.tex <==
% Some illegal space-saving macros
\parskip=3pt
\abovedisplayskip 3.0pt plus2pt minus2pt%
\belowdisplayskip \abovedisplayskip
\renewcommand{\baselinestretch}{0.98}

\newenvironment{packed_enum}{
\begin{enumerate}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}
{\end{enumerate}}

\newenvironment{packed_item}{
\begin{itemize}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{itemize}}

\newlength{\sectionReduceTop}
\newlength{\sectionReduceBot}
\newlength{\subsectionReduceTop}
\newlength{\subsectionReduceBot}
\newlength{\abstractReduceTop}
\newlength{\abstractReduceBot}
\newlength{\captionReduceTop}
\newlength{\captionReduceBot}
%\newlength{\nameReduceTop}
\newlength{\subsubsectionReduceTop}
\newlength{\subsubsectionReduceBot}

\newlength{\eqnReduceTop}
\newlength{\eqnReduceBot}

\newlength{\horSkip}
\newlength{\verSkip}

\newlength{\figureHeight}
\setlength{\figureHeight}{1.7in}

%\newlength{\figureFraction}
\setlength{\horSkip}{-.09in}
\setlength{\verSkip}{-.1in}
%\setlength{\figureFraction}{.195}


%
\setlength{\subsectionReduceTop}{-0.09in}
\setlength{\subsectionReduceBot}{-0.09in}
\setlength{\sectionReduceTop}{-0.10in}
\setlength{\sectionReduceBot}{-0.10in}
\setlength{\subsubsectionReduceTop}{-0.06in}
\setlength{\subsubsectionReduceBot}{-0.05in}
%
%
%\setlength{\figureHeight}{1.5in}
\setlength{\abstractReduceTop}{-0.05in}
\setlength{\abstractReduceBot}{-0.10in}
%
%

\setlength{\eqnReduceTop}{-0.05in}
\setlength{\eqnReduceBot}{-0.05in}

%\setlength{\nameReduceTop}{-0.05in}


\setlength{\captionReduceTop}{-0.12in}
\setlength{\captionReduceBot}{-0.12in}
%\setlength{\captionReduceBot}{-0.15in}

==> archive/tex/tab_results.tex <==
\begin{table*}[t]
    \begin{center}
        \scalebox{0.77}{%
            \begin{tabular}{
                p{0.18\columnwidth}
                ccccc
            }
            \toprule[\heavyrulewidth]
            \multirow{2}{*}{\textbf{Model}}
            & \multicolumn{1}{c}{\textbf{Task 1. Disamb.}}
            & \multicolumn{1}{c}{\textbf{Task 2. MM-Coref}}
            & \multicolumn{2}{c}{\textbf{Task 3. DST}}
            & \multicolumn{1}{c}{\textbf{Task 4. Generation}}\\            
            \cmidrule(r){2-2}
            \cmidrule(r){3-3}
            \cmidrule(r){4-5}
            \cmidrule(r){6-6}
                & Accuracy$\uparrow$
                & Coref F1$\uparrow$
                & Slot F1$\uparrow$
                & Intent F1$\uparrow$
                & BLEU$\uparrow$ \\            
            \midrule
            Baseline
                & \reportvalbrief{56.7}{0}
                & \reportvalbrief{79.3}{0}
                & \reportvalbrief{63.7}{0}
                & \reportvalbrief{1.9}{0}
                & \reportvalbrief{0.271}{0}\\            
            \bottomrule[\heavyrulewidth]
            \end{tabular}
        }
    \end{center}
    %\vspace*{-10pt}
        \caption{
        Summary of the baseline results.
        \textbf{(1) Multimodal Disambiguation (Disamb.)}, via classification
        \underline{accurac}y, 
        \textbf{(2) Multimodal Coreference Resolution (MM-Coref)}, via \underline{coref} prediction \underline{F1},
        \textbf{(3) Dialog State Tracking (DST)}, via \underline{slot} and \underline{intent} prediction \underline{F1},
        \textbf{(4) Response Generation} via \underline{BLEU}.
        $\uparrow$: higher is better, $\downarrow$: lower is better.
        }
        %\vspace*{\captionReduceBot}
    \label{tab:results}    
\end{table*}


==> archive_simmc_proposal.tex <==



\section{Motivation}

% 1. Brief recap of SIMMC 1.0
The Situated and Interactive Multimodal Conversaitional AI (SIMMC) challenge \cite{moon2020situated}, held as part of DSTC9 \cite{dstc9}, aimed to lay the foundations for the real-world assistant agents that can handle multimodal inputs, and perform multimodal actions.
Specifically, it provided the SIMMC corpora as a new benchmark dataset for studying task-oriented dialogs that encompass a situated multimodal user context in the form of a co-observed image or virtual reality (VR) environment.
The earlier SIMMC challenge saw a number of model submissions from participants, 
establishing a new set of state-of-the-art baselines for the multimodal task-oriented dialog systems on the SIMMC dataset.

% 2. Building upon it, we propose SIMMC 2.0, addressing the gaps
Building upon the success of the first SIMMC challenge \cite{moon2020situated}, we propose the Second SIMMC Challenge for the community to tackle and continue the effort towards building a successful multimodal assistant agent.
Specifically, we provide the newly collected dataset (SIMMC 2.0) designed to include a closer-to-real-world context for a fashion or furniture shopping scenario, moving away from the sanitized contexts present in the original SIMMC datasets.
To this end, SIMMC 2.0 presents assistant$\leftrightarrow$user task-oriented dialogs grounded on diverse photo-realistic VR renders of (synthetic) commercial stores.
These renderings include a number of referent items and serves as a proxy for real-world
scenarios.
This new dataset captures several interesting challenges such multimodal dialog state tracking, coreferences (``\textit{directly behind it}”, ``\textit{the one I mentioned}”), and disambiguation (``\textit{grey jacket to the right of the one I mentioned}”).

% 3. Summary; might be too verbose & repetitive so skip
%\textbf{In summary}, SIMMC 2.0 builds upon and extends the previous challenge, addressing the following main key challenges and gaps:
%\begin{itemize}
    %\item More complex multimodal contexts: 
    %\item Multimodal coreference resolution and dialog state tracking: 
    %\item Complex visual scenes: visually challenging problem
%\end{itemize}

%---------------------------------
\begin{figure}[t]
  \centering \includegraphics[width=1.0\columnwidth]{figures/overview.png}
  \vspace{-12pt}
  \caption{Illustration of a Situated Interactive Multimodal Conversation (SIMMC), which presents a task-oriented user$\leftrightarrow$assistant dialog grounded in a co-observed multimodal context. The newly collected SIMMC 2.0 dataset includes complex and photorealistic multimodal contexts, which poses more challenges for the Multimodal Coreference Resolution task (MM-Coref) and the Multimodal Dialog State Tracking task. } 
  \label{fig:teaser}
  \vspace{-10pt}
\end{figure}
%---------------------------------


\section{SIMMC Challenge 2.0}

We now detail the new multimodal conversational dataset (\refsec{subsec:dataset}) and propose 
three main sub-tasks for the challenge (\reftab{tab:tracks}, \refsec{subsec:tracks}).

\subsection{Problem Setup}

%\todo{paraphrase a bit more to avoid self-plagiarism}
The SIMMC challenge addresses the conversational scenarios where the virtual assistant shares a co-observed scene with a user in addition to the traditional communication that takes place in the form of natural language.
Following the SIMMC 1.0 dataset, we choose shopping experience as the domain for this study, as it often induces rich multimodal interactions around browsing visually grounded items.
We assume that the assistant agent has ground-truth meta information of every object in the scene, while users only observe those objects through the visual modality to describe and compose a request.
In addition, we allow users to physically navigate within each scene, which we simulate as multiple viewpoints updated at different time steps throughout each dialog.
Thus, entries to the SIMMC challenge 2.0 would need to understand the user utterance using both the dialog history and the state of the environment as multimodal context.

Note that our problem setup for co-observing assistant scenarios allows for more natural multimodal coreferences to be used as part of user-assistant conversations.
The existing literature in multimodal dialogs \cite{avsd-dstc7,avsd-dstc8,visdial,clevr-dialog,guesswhat,talk-the-walk} often posits the roles of a primary and secondary observer, \ie \textit{questioner} and \textit{answerer} similar to the Visual Question Answering \cite{vqa} tasks, hence showing a different distribution of language.
Our setup also extends many of the challenges studied in the previous literature on task-oriented dialog systems \cite{dstc2, sgd-dst, multiwoz, multiwoz2.1} (\eg DST, slot carryovers) to the unique multimodal settings.


\subsection{Description of Dataset}
\label{subsec:dataset}

\begin{table*}[t]
    \begin{center}
        \scalebox{0.9}{
        \setlength\tabcolsep{9pt}
        \begin{tabular}{p{0.28\textwidth}p{0.35\textwidth}p{0.25\textwidth}}
        \toprule[\heavyrulewidth]
        \textbf{Task Name}  & \textbf{Goal} & \textbf{Evaluation} \\
        \midrule
        1. Multimodal Coreference Resolution & Given user utterances with object mentions, resolve referent objects to their canonical ID(s) as defined by the catalog. & Coref Precision / Recall / F1 \\        
        \midrule        
        2. Multimodal Dialog State Tracking & Given user utterances, track user belief states across multiple turns. & Intent Accuracy,
Slot Precision / Recall / F1 \\
        \midrule
        3. Response Generation & Given user utterances, ground-truth APIs and ground-truth object IDs, generate Assistant responses or retrieve from a candidate pool. & Generation: BLEU, Perplexity, Human Evaluation (Naturalness, etc.); Retrieval: Accuracy@k, Entropy \\
        \bottomrule[\heavyrulewidth]
        \end{tabular}
        }
    \end{center}
    \vspace{-6pt} 
    \caption{\textbf{Proposed tracks and descriptions}}
    \vspace{-8pt} 
    \label{tab:tracks}
\end{table*}


The SIMMC 2.0 dataset assumes the scenario where a user is interacting with a conversational assistant to obtain recommendations for a furniture or a fashion item.
The dialogs were collected through a two-phase pipeline (multimodal dialog simulation \& manual human paraphrase), minimizing the annotation overheads (time and cost).
This approach extends the popular machine$\leftrightarrow$human collaborative dialog collection approaches \cite{sgd-dst, shah2018building} to the multimodal settings.

\textbf{Phase 1}: We generate synthetic dialog flows using a dialog simulator that conditions on various VR scenes for fashion and furniture, produced by a scene simulator.
The scene simulator generates a diverse set of scene snapshots that serve as multimodal context for the conversations. This is done using publicly available digital assets, re-arranging them programmatically at random to create scenes, and capturing a view from a random camera position within the scene. 

The dialog simulator then takes these generated scenes along with the meta information (objects, locations, and attributes) to create a dialog flow between a user and an assistant, following an agenda-based dialog simulator approach \cite{schatzmann2007agenda}.
Each agenda describes a high-level sequence of shopping scenarios (\eg \texttt{BROWSE} $\rightarrow$ \texttt{GET\_INFO} $\rightarrow$ \texttt{REFINE}).
The simulated dialog flows consist of NLU/NLG intents (\eg \texttt{REQUEST:GET}, \texttt{CONFIRM:ADD\_TO\_CART}), slots (\eg color, pattern), and object references, following the ontology developed for SIMMC 1.0 \cite{moon2020situated}.

\textbf{Phase 2}: The simulated dialog flows are then paraphrased by human annotators. This helps us draw utterances from the natural language distribution, as expected in a real world application. For this annotation effort, we designed a tool that displays a multimodal scene (generated VR scene screenshot) and a simulated dialog flow, and asked the human annotators to paraphrase the utterance ensuring that critical information such as objects and attributes is retained. An example dialog is shown in \reffig{fig:example}.

\begin{table}[h]
    \begin{center}
        \scalebox{0.92}{
        \begin{tabular}{lccc}
        \toprule[\heavyrulewidth]
        Total \# dialogs & 11,244 \\
        Total \# utterances & 117,236 \\
        Total \# scenes & 3,133 \\
        Avg \# words per user turns 	& 12 \\
        Avg \# words per assistant turns &	13.7 \\
        Avg \# utterances per dialog 	& 10.4 \\
        Avg \# objects mentioned per dialog &	4.7 \\
        Avg \# objects in scene per dialog &	19.7 \\
        \bottomrule[\heavyrulewidth]
        \end{tabular}
        }
    \end{center}
    \vspace{-10pt} 
    \caption{\textbf{SIMMC 2.0 Dataset Statistics}}
    \vspace{-10pt}   
    \label{tab:datasets_statistics}
\end{table}

We collected a total of 11,244 dialogs (117,236 utterances), with the fine-grained ground-truth dialog labels (NLU/NLG/Coref) already in place.
Table~\ref{tab:datasets_statistics} shows the statistics of the dataset.

\noindent
\textbf{Differences between SIMMC 1.0 and 2.0}.
The key differences are (illustrated in \reffig{fig:teaser}):

\noindent
(a) The multimodal context in SIMMC 1.0 consists of either co-observed images or VR environment,
which are simplistic and sanitized in comparison to real-world scenarios.
For instance, the VR environment in SIMMC-Furniture comprises three slots (left, center, right) 
to populate the catalog items, thus limiting the complexity of referential or disambiguation language.
In contrast, conversations in SIMMC 2.0 are grounded in photo-realistic scene renderings of
commercial stores that are cluttered and thus closely represent the real-world contexts.

\noindent
(b) The number of objects in the multimodal context for SIMMC 1.0 at any turn is capped at 3
compared to $19.7$ on average for SIMMC 2.0.
This allows for richer coreferences, referential expressions, and disambiguation scenarios, 
elevating the role of dialog.

\noindent
(c) Many of the objects in each scene are only partially observed (\eg, blocked by different items or shelves, out of POV frame), which reflects real-world scenes but poses a more challenging problem for the computer vision module.

\noindent
\textbf{Data format}:
The SIMMC 2.0 data will be provided in the similar format as the earlier version of the dataset, to make it easier for participants to leverage the benchmark models publicly available \cite{moon2020situated}, or augment it with the previous version of the dataset for pretraining, etc.
The raw pixel images of each scene as well as the pre-computed visual embeddings (via a popular CV model) will be provided, to make it easier to use the dataset.

\subsection{Challenge Tasks}
\label{subsec:tracks}

We invite participants to model multimodal conversational agents adept at replicating humans for this dataset and enable deep shopping scenarios as a result.
The entries to the SIMMC 2.0 challenge would thus need to have a strong computer vision capability to consume raw images we provide, and a multimodal conversational reasoning capability to understand both the dialog and the visual contexts. 
Specifically, we propose three sub-tasks and evaluation metrics addressing the challenges in the multimodal conversational reasoning (summarized in \reftab{tab:tracks}).
A script for calculating these metrics will be provided with the dataset.

\subsubsection{Multimodal Coreference Resolution (MM-Coref)}
For this task, we aim to resolve referential mentions in user utterances to their canonical object IDs as defined for each scene.
These mentions can be resolved through (1) the dialog context (\eg A: ``\textit{\underline{This shirt} comes in XL and is \$29.}" $\rightarrow$ U: ``\textit{Please add \underline{it} to cart.}", or (2) the multimodal context (\eg U: ``\textit{How much is that \underline{red shirt}?}"), or (3) both (\eg U: ``\textit{How much is \underline{the one} next to \underline{the one you mentioned}?}").

Participants will be provided with ground-truth bounding boxes defining each object ID.
The performance will mainly be measured for its F1 score.

\subsubsection{Multimodal Dialog State Tracking (MM-DST)}
Following the earlier challenge, we extend the traditional notion of the unimodal dialog state tracking (DST) problem and propose MM-DST as a main sub-task where slots are grounded on the coexisting multimodal context, which requires handling of multimodal objects (as opposed to textual tokens) as part of dialog states.

\subsubsection{Assistant Response Generation}
The goal of this task is to generate Assistant responses or retrieve from a candidate pool, given user utterances, ground-truth APIs and object IDs.
While we assume the assistant agent has the ground-truth meta information on each object, each response needs to naturally describe the referent objects \textit{as observed and understood} by the user through the co-observed scene or the dialog context (\eg \texttt{INFORM:RECOMMEND (OBJ\_ID: 3)} $\rightarrow$ A: ``\textit{I recommend the blue shirt directly behind the brown jacket.}". 


\section{Organizers}

\noindent Seungwhan Moon; \texttt{shanemoon@fb.com}

\noindent Satwik Kottur; \texttt{skottur@fb.com}

\noindent Paul A. Crook; \texttt{pacrook@fb.com}

\noindent Ahmad Beirami; \texttt{beirami@fb.com}

\noindent Eunjoon (EJ) Cho; \texttt{ejcho@fb.com}

\noindent Babak Damavandi; \texttt{babakd@fb.com}

\noindent Alborz Geramifard; \texttt{alborzg@fb.com}

\noindent Rajen Subba; \texttt{rasubba@fb.com}


\bibliography{bibliography}
\bibliographystyle{plain}
% \bibliographystyle{acl_natbib}
\vfill
\pagebreak

\input{tex/supplementary.tex}

